Ex-post Individually Rational Bayesian Persuasion

In the Bayesian persuasion model, a sender can convince a receiver to choose an alternative action to the one originally preferred by the receiver. A crucial assumption in this model is the sender's commitment to a predetermined information disclosure policy (signaling scheme) and the receiver's trust in this commitment. However, in practice, it is difficult to monitor whether the sender adheres to the disclosure policy, and the receiver may refuse to follow the persuasion due to a lack of trust. Trust becomes particularly strained when the receiver knows that the sender will incur obvious losses when truthfully following the protocol. In this work, we propose the notion of ex-post individually rational (ex-post IR) Bayesian persuasion: after observing the state, the sender is never asked to send a signal that is less preferred than no information disclosure. An ex-post IR Bayesian persuasion policy is more likely to be truthfully followed by the sender, thereby providing stronger incentives for the receiver to trust the sender. Our contributions are threefold. First, we demonstrate that the optimal ex-post IR persuasion policy can be efficiently computed through a linear program, while also offering its geometric characterization. Second, we show that surprisingly, for non-trivial classes of games, the requirement of ex-post IR constraints does not incur any cost to the sender's utility. Finally, we compare ex-post IR Bayesian persuasion to other information disclosure models that ensure different notions of credibility.

==> comparison.tex <==
\section{Comparison of the sender's optimal utility}\label{section:compare}
In this section, we compare the sender's expected utility under different credibility requirements. We consider four information transmission models with different credibility levels: Bayesian persuasion, ex-post IR Bayesian persuasion, 
 credible persuasion~\cite{lin2022credible}, and cheap talk~\cite{crawford1982strategic}. In many previous works about Bayesian persuasion with partial commitment, such as \cite{min2021bayesian,lin2022credible}, the optimal sender utility achieved by their model is between the Bayesian persuasion and cheap talk. Therefore, it is natural to compare the sender's optimal utility of our ex-post IR Bayesian persuasion with the commitment power of Bayesian persuasion and cheap talk. Besides, since our model considers the credibility of the sender, we compare the ex-post IR Bayesian persuasion to another model called \emph{credible persuasion} in the paper by \cite{lin2022credible}, which also considers the credibility of the sender.

%We will compare four information transmission models: Bayesian persuasion, ex-post IR Bayesian persuasion, credible persuasion, and cheap talk. 
Given the sender's utility $v$, receiver's utility $u$, the optimal sender utilities gained in these four models is the functions of prior $\mu_0$ and denoted as $V_{\textsc{BP}}(\mu_0)$, $V_{\textsc{expost}}(\mu_0)$, $V_{\textsc{credible}}(\mu_0)$, $V_{\textsc{cheap}}(\mu_0)$. We formally give the definition that the optimal sender utility achieved in one information transmission model is better than the optimal sender utility achieved in another information transmission model.
\begin{definition}
Consider two information transmission model $X, Y$. If for any $v,u,\mu_0$, we have $V_X(\mu_0)\ge V_Y(\mu_0)$, we say the optimal sender utility achieved in $X$ is better than the optimal sender utility achieved in $Y$, which is denoted by $V_X\succeq V_Y$.
\end{definition}

% Next we assume $\cref{sorted}$ hold and we will show that $V^{\mathrm{expostBP}}\succeq V^{\mathrm{Cheaptalk}}$. Therefore, we can also put our model in the scope of Bayesian persuasion with partial commitment and compare it to credible persuasion. We give a brief introduction to the credible persuasion.

Next, we compare the optimal sender utility of the aforementioned four information transmission models. Before that, We give a brief introduction to credible persuasion.

\paragraph{Credible persuasion} The interaction between the sender and the receiver goes on as follows:
\begin{enumerate}    
    \item sender chooses a signaling scheme $\phi$. Different from the Bayesian persuasion, the receiver cannot observe the signaling scheme;
    \item sender observes a realized state of nature $\theta\sim\mu_0$;
    \item sender draws a signal $s\in S$ according to the distribution $\phi_{\theta}$ and sends it to the receiver;
    \item receiver observes the signal $s$. Different from the Bayesian persuasion, the receiver can also observe the marginal distribution of signals induced by $\phi$. 
    
    % \swcomment{should we mention this is the marginal distribution?}
    \item The receiver chooses an action based on both the signal $s$ and the distribution of signals.
\end{enumerate}

Their notion of credibility is captured by the restriction that the receiver can only see the distribution of the signal induced by a signaling scheme $\phi$ instead of the whole signaling scheme. The receiver can not distinguish the signaling schemes that induce the same distribution of signals as $\phi$. Denote the set of such signaling schemes $D(\phi)$. They require when the sender chooses a signaling scheme $\phi$, it has no profitable deviation in $D(\phi)$.

Now we are ready to present our comparison results. We show that both ex-post IR Bayesian persuasion and credible persuasion are partial commitment models between Bayesian persuasion and cheap talk. Then we show that in some games, the commitment power of ex-post IR Bayesian persuasion is stronger than the commitment power of credible persuasion.  While in some other games, the commitment power of credible persuasion is stronger than the commitment power of ex-post IR Bayesian persuasion. The results are summarized in \cref{thm:compare}. 

\begin{theorem}\label{thm:compare}
The ranking of the optimal sender's utility is as follows:
\begin{enumerate}
    \item $V^{\mathrm{BP}}\succeq V^{\mathrm{credible}},V^{\mathrm{expostBP}}\succeq V^{\mathrm{cheaptalk}}$.
    \item  There exists $v,u$ such that for any $\mu_0$, \[V^{\mathrm{credible}}(\mu_0)\ge V^{\mathrm{expostBP}}(\mu_0).\]
    \item  There exists $v,u$ such that for any $\mu_0$, \[V^{\mathrm{expostBP}}(\mu_0)\ge V^{\mathrm{credible}}(\mu_0).\]
\end{enumerate} 
\end{theorem}
The first part of \cref{thm:compare} that ex-post IR Bayesian persuasion and credible persuasion are partial commitment models between Bayesian persuasion and cheap talk. The second part of \cref{thm:compare} that the commitment power of ex-post IR Bayesian persuasion and credible persuasion differs in different cases based on a series of lemma that show when the optimal sender utility of ex-post IR Bayesian persuasion or credible persuasion is the same as the optimal sender utility of Bayesian persuasion. Then we can construct examples when one model's optimal sender utility is equal to the optimal sender utility of Bayesian persuasion and the other model's optimal sender utility is strictly smaller than the optimal sender utility of Bayesian persuasion.

At last, we claim that \cref{sorted} is the key to make sure that the ex-post IR Bayesian persuasion is between Bayesian persuasion and cheap talk. Actually, we can give an example that if \cref{sorted} doesn't hold, the optimal sender utility achieved by the ex-post IR Bayesian can be worse than the utility achieved by the cheap talk. In other words, there exists $v,u,\mu_0$ such that $V^{\mathrm{cheaptalk}}(\mu_0)>V^{\mathrm{expostBP}}(\mu_0)$. Our example is based on the following  \cref{lem:cheapnogap} that shows when there is no sender utility gap between the Bayesian persuasion and cheap talk.
\begin{lemma}\label{lem:cheapnogap}\cite{lipnowski2020equivalence}
  If the expected sender utility $\hat{v}$ is continuous, for any $v,u,\mu_0$, $V^{\mathrm{BP}}(\mu_0)=V^{\mathrm{Cheaptalk}}(\mu_0)$.
\end{lemma}
Then we can construct an example that the optimal sender utility gained by cheap talk is the same as the optimal sender utility gained by the Bayesian persuasion while the optimal sender utility gained by ex-post IR Bayesian persuasion is strictly smaller than the optimal sender utility gained by the Bayesian persuasion.

\begin{example}\label{ex: ch>expost}
    Consider $A=\{a_1,a_2,a_3,a_4,a_5\}$ and $\theta=\{\theta_1,\theta_2\}$, the sender utility $v$ and the receiver utility $u$ is as follows.
\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|}
\hline
  & $\theta_1$ & $\theta_2$ \\ \hline
$a_1$ & 10 & 0 \\ \hline
$a_2$ & -2 & 3 \\ \hline
$a_3$ & 1 & 1 \\ \hline
$a_4$ & 3 & -2 \\ \hline
$a_5$ & 0 & 10 \\ \hline
\end{tabular}
\qquad
\begin{tabular}{|l|l|l|}
\hline
  & $\theta_1$ & $\theta_2$ \\ \hline
$a_1$ & -4 & 21 \\ \hline
$a_2$ & 0 & 20 \\ \hline
$a_3$ & 12 & 12 \\ \hline
$a_4$ & 20 & 0 \\ \hline
$a_5$ & 21 & -4 \\ \hline
\end{tabular}
\caption{The utility of sender and receiver in \cref{ex: ch>expost}}
\label{tab:compare}
\end{table}

For any $\mu_0$ that $\mu_0(\theta_1)\in(\frac{2}{5},\frac{3}{5})$, $a^*(\mu_0)=a_3$. The optimal ex-post IR signaling scheme is no communication and $V^{\mathrm{expostBP}}(\mu_0)=1$. $\hat{v}$ is continuous so the optimal sender utility of cheap talk is equal to the optimal sender utility of Bayesian persuasion. We have $V^{\mathrm{Cheaptalk}}(\mu_0)=2$. Therefore, $V^{\mathrm{Cheaptalk}}(\mu_0)>V^{\mathrm{expostBP}}(\mu_0)$ for any $\mu_0\in(\frac{2}{5},\frac{3}{5})$.
\end{example}

==> conclusion.tex <==
\section{Conclusion}
In this paper, we studied ex-post IR Bayesian persuasion, a novel Bayesian persuasion model with restricted commitment power in which the sender must commit to a signaling scheme that the sender's ex-post utility given a realized world state and signal is always no worse than the utility he can gain by no communication given the same world state. We show that the ex-post IR constraint is a linear constraint; hence, linear programming can still solve the optimal ex-post IR signaling scheme. Our main results give broad conditions when there is no utility gap for the sender between the optimal signaling scheme and the optimal ex-post IR signaling scheme. In the binary state case, we show that the optimal signaling scheme is also ex-post IR if and only if the smoothed quasiconcave closure of the sender's expected utility function is concave. We also show that, in the general case, if the Bayesian persuasion instance is a trading game or is modeled as a credence goods market, then the optimal signaling scheme is ex-post IR. We also extend the credence goods market model to a class of games that satisfy the cyclical monotonicity and weak supermodularity in logarithmic form. We show the greedy signaling scheme is ex-post IR in this class of games, and hence, the gap between the optimal signaling scheme and optimal ex-post IR signaling scheme can be controlled by the gap between the optimal signaling scheme and the greedy signaling scheme. At last, we show that, in the sense of the sender's optimal utility, our model is an information transmission model between Bayesian persuasion and cheap talk.
\paragraph{Future work} We provide additional ideas for future work. There are many interesting technical questions that arise from this persuasion model. Since we only give a necessary and sufficient condition in the binary state case to determine whether the optimal signaling scheme is ex-post IR. A natural question is, can we extend our result in the binary state case to the case that the number of world states is higher? Or can we discover some general structure of the sender's utility function and receiver's utility function to make sure the optimal signaling scheme is ex-post IR?  Also, in \cref{cor:greedy}, we use a greedy signaling scheme to bound the gap led by the ex-post IR constraint. There are many known results about the approximate ratio of greedy algorithms. It seems promising to explore further when the greedy signaling scheme is approximately optimal. It is of interest to see whether there are other tools rather than greedy signaling schemes that can help to characterize the gap. Finally, though our paper focuses on the impact on the sender's utility, it is interesting to consider the impact on the receiver's utility and social welfare with the existence of the ex-post IR constraint.

